Parameterized Quantum Query Algorithms for Graph Problems

In this paper, we consider the parameterized quantum query complexity for graph problems. We design parameterized quantum query algorithms for $k$-vertex cover and $k$-matching problems, and present lower bounds on the parameterized quantum query complexity. Then, we show that our quantum query algorithms are optimal up to a constant factor when the parameters are small.

==> missing_proofs.tex <==
\section{Omitted Proofs} \label{sec:ommitted_proof}

\subsection{Proof of Lemma \ref{lem:find_k_restricted_maximal_matching}} \label{subsec:omit_proof_from_threshold_matching}

\begin{proof}[Proof of Lemma \ref{lem:find_k_restricted_maximal_matching}]
% It remains to analyze the quantum query complexity of Algorithm \ref{alg:quantum_threshold_maximal_matching}.
% We first consider the case where this procedure outputs $\bot$.
% We assume that the size of $E_M$ is $s$ 
% Let $s$ denote the size of $E_M$ after the execution of the while loop in \texttt{QuantumThresholdMaximalMatching}.
% \ryuheidel{We first consider the following procedure.
% We begin with an empty set $M$.
% We repeatedly use the search procedure to find an edge $e$ whose endpoints are both in $V(G) \setminus V(M)$ and add $e$ to $M$.}

% \ryuheidel{The search procedure finds an edge
% with expected $8 \sqrt{n^2 / t}$ queries
% if there are $t > 0$ edges whose endpoints are both in $V(G) \setminus V(M)$
% and otherwise runs forever.
% We note that the procedure \texttt{QuantumThresholdMaximalMatching} (Algorithm \ref{alg:quantum_threshold_maximal_matching}) is obtained by stopping the above procedure after it uses $96 n \sqrt{k + 1}$ queries.}


We first consider Algorithm~\ref{alg:quantum_threshold_maximal_matching} without the limit of queries, which is described as Algorithm \ref{alg:quantum_threshold_matching_run_forever}.
This algorithm does not terminate.
We will show that the expected number of queries until $M$ becomes a maximal matching or a matching of size $k+1$ is at most $16n\sqrt{k+1}$.
% Then, with the limit $96n\sqrt{k+1}$ of queries, the algorithm outputs a maximal matching or a matching of size at least $k+1$ with probability at least $5/6$.
Then, even if we limit the number of queries to $96n\sqrt{k+1}$, the algorithm outputs a maximal matching or a matching of size at least $k+1$ with probability at least $5/6$.

\begin{algorithm}[H]
    $M \gets \emptyset$ \\
    \While{true} {
        Apply Las Vegas-type Grover's search algorithm to find an edge $e$ whose endpoints are both in $V(G) \setminus V(M)$ \\
        $M \gets M \cup \{e\}$
    }
    \caption{The procedure \texttt{QuantumThresholdMaximalMatching} (Algorithm \ref{alg:quantum_threshold_maximal_matching}) without the limit of queries} \label{alg:quantum_threshold_matching_run_forever}
\end{algorithm}

Recall that the Las~Vegas-type Grover's algorithm in Lemma~\ref{lem:grover_expected_find} has a finite expected number of queries. This means that the Las~Vegas-type Grover's algorithm finds an edge with probability 1 if it exists.
Hence, in the non-halting algorithm, $M$ becomes a maximal matching of $G$ after finite number of queries with probability 1.
Let $M^*$ be a random variable corresponding to the maximal matching found by the non-halting algorithm.
Let $T=|M^*|$.
Then, by Lemma~\ref{lem:grover_expected_find}, for finding an $i$-th edge of $M^*$, the Las~Vegas-type Grover's algorithm has a expected quantum query complexity at most $8\sqrt{\frac{n^2}{T-i+1}}$, since there exist at least $T-i+1$ edges in vertex pairs of $V(G)\setminus V(M)$.
Hence, the expected number of queries until $M$ becomes a maximal matching or a matching of size $k+1$ is at most


% \ryuheidel{
% We assume that the above procedure finds a matching of size $s$ at some point in time.
% When we search for the $i$--th edge, 
% there exist at least $s + 1 - i$ edges whose endpoints are both in $V(G) \setminus V(M)$.
% Thus, by Lemma \ref{lem:grover_expected_find}, we find the $i$--th edge with expected at most $\displaystyle 8 \sqrt{\frac{n^2}{s + 1 - i}}$ queries.
% Then, the expected total number of queries used by the search procedure to find all $s$ edges is bounded by }
\begin{align*}
\sum_{i = 1}^{\min\{T,\,k+1\}} 8 \sqrt{\frac{n^2}{T-i+1}} \leq
\sum_{i = 0}^{k} 8 \sqrt{\frac{n^2}{i+1}} \le
8 n \int_{0}^{k+1} \frac{dx}{\sqrt{x}} = 16 n \sqrt{k+1}.
\end{align*}
This completes the proof of Lemma~\ref{lem:find_k_restricted_maximal_matching}.
\end{proof}

% \ryuheidel{
% If the above procedure finds a matching of size $s$ at some point in time, then it finds a matching of size at least $s$ with probability at least $5/6$ after it uses $6$ times the expected total number of queries.}

% Furthermore, 
% if the above procedure finds a maximal matching of size $s \leq k$,
% it finds a matching of size $s$ with probability at least $5/6$
% % in $96 n \sqrt{k + 1}$ queries
% after it uses $6$ times the expected total number of queries.
% with probability at least $5/6$.
% Thus, if the above algorithm finds a maximal matching of size $s \leq k + 1$, 
% \texttt{\textup{QuantumThresholdMaximalMatching}} (Algorithm \ref{alg:quantum_threshold_maximal_matching})

% \ryuheidel{
% The procedure \texttt{QuantumThresholdMaximalMatching} (Algorithm \ref{alg:quantum_threshold_maximal_matching}) is obtained by stopping the above procedure after it uses $96 n \sqrt{k + 1}$ queries.
% Therefore, with probability at most $5/6$, the procedure
% \texttt{QuantumThresholdMaximalMatching} outputs a matching of size at least $k + 1$ or a maximal matching, which completes the proof.}
% % after the expected number $\displaystyle \sum_{i = 1}^{s} 8 \sqrt{\frac{n^2}{s + 1 - i}} \leq 8 n \int_{0}^{s} \frac{dx}{\sqrt{x}} = 16 n \sqrt{s}$ queries.
% % Next we consider the case where this procedure does not output $\bot$.
% % \begin{align*}
% % \sum
% % \end{align*}
% \end{proof}

\subsection{Proofs of Lemma \ref{lem:vertex_cover_while_loop} and Theorem \ref{thm:quantum_query_best_algorithm_vertex_cover}} \label{subsec:omit_proof_from_vertex_cover}

\begin{proof}[Proofs of Lemma \ref{lem:vertex_cover_while_loop}]
In the same way as the proof of Lemma \ref{lem:find_k_restricted_maximal_matching}, we consider the while loop of the procedure \texttt{Quantum $k$-Vertex Cover} without the limit of queries, which is described as Algorithm \ref{alg:quantum_vertex_cover_run_forever}.
We will show that the expected total number of queries until the properties (i) and (ii) hold is at most $32 k \sqrt{(k + 1) n}$.
Then, in Algorithm \ref{alg:quantum_vertex_cover_run_forever}, after the search algorithm used $192 k \sqrt{(k + 1) n}$ queries, the properties (i) and (ii) hold with probability at least $5/6$.

% With probability $5/6$, we find all edges after $6$ times the expected total number of queries.
% Furthermore, after we found all $s$ edges, the properties (i), (ii) hold.
% Therefore, after the execution of the while loop in the procedure \texttt{Quantum $k$-Vertex Cover},
% the properties (i), (ii) hold with probability at least $5/6$.

\begin{algorithm}[t]
    $U \gets \emptyset$, $E' \gets \emptyset$, $k' \gets k$ \\
    For $v \in V(M)$, $N_v \gets \emptyset$ \\
    \While{true} {
        Apply Las Vegas-type Grover's search algorithm to find an edge $e \in \{ (v, u) \mid v \in V(M) \setminus U \text{ and } u \in V(G) \} \setminus E'$  \label{line:quantum_vertex_cover_2_run_forever} \\
        $E' \gets E' \cup \{ (v, u) \}$ \\
        $N_v \gets N_v \cup \{ u\}$ \\
        \If{$|N_v| > k$} {
            $U \gets U \cup \{v\}$, $k' \gets k' - 1$ \\
        }
        \If{$u \in V(M)$} {
            $N_u \gets N_u \cup \{ u \}$ \\
            \If{$|N_u| > k$} {
                $U \gets U \cup \{u\}$, $k' \gets k' - 1$ \\
            }
        }
    }
    \caption{The while loop of the procedure \texttt{Quantum $k$-Vertex Cover} (Algorithm \ref{alg:quantum_vertex_cover}) without the limit of queries} \label{alg:quantum_vertex_cover_run_forever}
\end{algorithm}

Let $E'^{*}$ (resp. $U^*$) is a random variable corresponding to $E'$ (resp. $U$) found by the non-halting algorithm.
Let $T = |E'^{*}|$.
Then, for finding an $i$-th edge of $E'^{*}$, the Las Vegas-type Grover's algorithm has a expected quantum query complexity of at most $8 \sqrt{\frac{2 k n}{T - i + 1}}$, since there exist at least $T - i + 1$ edges in the set $\{ (v, u) \mid v \in V(M) \setminus U \text{ and } u \in V(G) \} \setminus E'$.
Note that we have $|V(M) \setminus U| \leq 2 k$, and then the size of the set $\{ (v, u) \mid v \in V(M) \setminus U \text{ and } u \in V(G) \}$ is at most $2 k n$.
% We assume that this procedure finds $s$ edges at some point in time.
% We also assume that, after we found $s$ edges, we have $\{ (v, u) \mid v \in V(M) \setminus U \text{ and } u \in V(G) \} \setminus E' = \emptyset$.
% When we search for the $i$--th edge, 
% there exist at least $s + 1 - i$ edges with one endpoint in $V(M) \setminus U$.
% Note that we have $|V(M) \setminus U| \leq 2 k$, and then the size of the search space is at most $2 k n$.
% Thus, by Lemma \ref{lem:grover_expected_find}, we find the $i$--th edge with expected at most $\displaystyle 8 \sqrt{\frac{2 k n}{s + 1 - i}}$ queries.
% Then, the expected total number of queries used by the search procedure to find all $s$ edges is bounded by 
Hence, the expected number of queries until the properties (i) and (ii) hold is at most
\begin{align*}
\sum_{i = 1}^{T} 8 \sqrt{\frac{2 k n}{T - i + 1}} \leq 8 \sqrt{2 k n} \int_{0}^{T} \frac{dx}{\sqrt{x}} = 16 \sqrt{2 k n T}.
\end{align*}
Note that, in Algorithm \ref{alg:quantum_vertex_cover_run_forever}, when $\{ (v, u) \mid v \in V(M) \setminus U \text{ and } u \in V(G) \} \setminus E' = \emptyset$, the properties (i) and (ii) hold.
Furthermore, we have $T \leq |V(M)| \cdot (k + 1) \leq 2 k (k + 1)$.
Then, the expected number of queries until the properties (i) and (ii) hold is at most $32 k \sqrt{(k + 1) n}$.
This completes the proof of Lemma \ref{lem:vertex_cover_while_loop}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:quantum_query_best_algorithm_vertex_cover}]
By Lemmas \ref{lem:find_k_restricted_maximal_matching} and \ref{lem:vertex_cover_while_loop}, the total number of queries used in the procedure \texttt{Quantum $k$-Vertex Cover} is $O(\sqrt{k}n + k^{3/2}\sqrt{n})$.
Then, it remains to show that \texttt{Quantum $k$-Vertex Cover} correctly find a vertex of size at most $k$ with probability at least $2/3$.

We say that the procedure \texttt{Quantum $k$-Vertex Cover} fails if one of the following conditions holds.
\begin{itemize}
\item The procedure \texttt{QuantumThresholdMaximalMatching} in Line \ref{line:quantum_kernelization_1} outputs a matching of size at most $k$, and the matching is not maximal.
\item After the execution of the while loop in the procedure \texttt{\textup{Quantum $k$-Vertex Cover}},
the properties at least one of (i) and (ii) in Lemma \ref{lem:vertex_cover_while_loop} does not hold.
\end{itemize}
By Lemmas \ref{lem:find_k_restricted_maximal_matching} and \ref{lem:vertex_cover_while_loop}, 
the procedure \texttt{Quantum $k$-Vertex Cover} fails with probability at most $1/3$.
Therefore, we only need to show that, if \texttt{Quantum $k$-Vertex Cover} does not fail, the procedure \texttt{Quantum $k$-Vertex Cover} determines whether the input graph $G$ contains a vertex cover of size at most $k$.

Now, we only consider the case where the procedure \texttt{Quantum $k$-Vertex Cover} does not fail.
First, we prove the following invariants at the beginning of any iteration of the while loop.
\begin{itemize}
\item The instance $(G - U, k')$ is equivalent to the input instance $(G, k)$.
\item Every vertex in $U$ must be in every vertex cover of size at most $k$.
\end{itemize}
Now, assume that the invariants hold true at the beginning of an iteration of the while loop.
By Observation \ref{obs:vertex_cover_kernelization}, 
if the degree of a vertex $v \in V(M)$ is more than $k$, then the instance $(G - U, k')$ is equivalent to the instance $(G - (U \cup \{v\}), k' - 1)$.
Note that we have $k \geq k'$.
% Note that this is the same argument used in \textbf{Reduction Rule 2} in the kernelization algorithm of Buss--Goldsmith.
Hence, the invariants remain true.

Next, we show that, after the execution of the for loop in Line \ref{line:quantum_vertex_cover_4}, every vertex cover in $G'$ is a vertex cover in $G - U$.
Every edge in $G$ has at least one endpoint in $V(M)$, since $M$ is a maximal matching.
This yields that, after the execution of the while loop, we have $E(G - U) \subseteq E'$.
% Then, after the execution of the for loop in Line \ref{line:quantum_vertex_cover_4}, $G'$ is the graph obtained by removing isolated vertices from the graph $G - U$, which completes the proof.
Hence, after the execution of the for loop in Line \ref{line:quantum_vertex_cover_4}, we have $G' = G - U$.

It remains to show that our quantum algorithm has time complexity $\tilde{O}(\sqrt{k}n + k^{3/2}\sqrt{n} + 1.2738^k)$.
First, the part of the quantum query kernelization has time complexity $\tilde{O}(\sqrt{k}n + k^{3/2}\sqrt{n})$.
Note that time complexity of Grover's search algorithm has a $\log (n)$ factor compared to its query complexity (see e.g., \cite[Section 2.4]{apers2021quantum}).
Here, the number of edges in the obtained subgraph $G'$ is $O(k^2)$,
since the size of $V(M)$ is at most $2 k$ and every non-removed vertex in $V(M)$ has degree at most $k$.
Now, we remove isolated vertices from $G'$ and then the number of vertices in $G'$ becomes $O(k^2)$.
Then, we can solve the {\sc $k$-vertex cover} problem for the instance $(G',  k')$ by the classical algorithm of Chen--Kanj--Xia \cite{chen2010improved} in time $O(1.2738^k)$.
This completes the proof of Theorem \ref{thm:quantum_query_best_algorithm_vertex_cover}.
\end{proof}

% \subsection{Proof of Theorem \ref{thm:upper_bound_of_k_matching}} \label{subsec:omit_proof_from_matching}

% \subparagraph*{Query Complexity of \texttt{Quantum $k$-Matching}}
% First, we analyze the query complexity of the procedure \texttt{Quantum $k$-Matching}.
% By Lemma \ref{lem:find_k_restricted_maximal_matching}, the number of queries in Line \ref{line:quantum_matching_0} is $O(\sqrt{k} n)$.
% Furthermore, the number of queries used in Line \ref{line:quantum_maching_1} is $O(k^2)$ and the number of queries used in Line \ref{line:quantum_maching_2} is $O(k \sqrt{n \log k})$, since we have $|V(M)| \leq 2 k$.
% The number of iterations of the outer while loop is bounded by $k$, since the size of the current matching $M$ increases by $1$ in a single iteration of the outer while loop.
% Then, the number of queries used in Line \ref{line:quantum_maching_5} is $O(k \sqrt{n \log k})$.
% Furthermore, the number of queries used in Lines \ref{line:quantum_maching_3} and \ref{line:quantum_maching_4} is $O(k^2)$ since we have $|V(M)| \leq 2 k$.
% Therefore, the total number of queries used in the procedure \texttt{Quantum $k$-Matching} is $O(\sqrt{k}n + k^2)$.

% \subparagraph*{Bounding the error probability of \texttt{Quantum $k$-Matching}}
% We say that the procedure \texttt{Quantum $k$-Matching} fails if one of the following conditions holds.
% \begin{itemize}
% \item[(i)] The procedure \texttt{QuantumThresholdMaximalMatching} in Line \ref{line:quantum_matching_0} outputs a matching of size at most $k$ that is not a maximal.
% \item[(ii)] The search procedure in Lines \ref{line:quantum_maching_2} and \ref{line:quantum_maching_5} does not find a vertex $u$ in $V(G) \setminus (V(M) \cup N_v)$ that are adjacent to $v$ although there exists such a vertex $u$.
% \end{itemize}

% By Lemma \ref{lem:find_k_restricted_maximal_matching}, the condition (i) holds with probability at most $1/6$.
% By Lemma \ref{lem:grover_stop_approx}, a call of search procedure fails to find a vertex, although there exists a vertex, with probability at most $O(1/k)$.
% In the whole run of the procedure \texttt{Quantum $k$-Matching}, the number of search procedure calls is $O(k)$.
% Then, by taking the union bound over the whole run of \texttt{Quantum $k$-Matching}, we obtain that the condition (ii) holds with probability at most constant.
% Therefore, the procedure \texttt{Quantum $k$-Matching} fails with probability at most $1/3$.

% \subparagraph*{Correctness of \texttt{Quantum $k$-Matching}}
% Now, we show that, if \texttt{Quantum $k$-Matching} does not fail, the procedure \texttt{Quantum $k$-Matching} determines whether the input graph $G$ has a matching of size at least $k$.
% Then, we only consider the case where the procedure \texttt{Quantum $k$-Matching} does not fail.
% Here, for each $v \in V(M)$, let $N_M(v)$ denote $\{u \in V(G) \setminus V(M) \mid (v, u) \in E(G) \}$, and let $E_M(v)$ denote $\{(v, u) \in E(G) \mid u \in N_M(v) \}$.

% First, we show that the following conditions hold at the beginning of any iteration of the while loop in Line \ref{line:qunatum_matching_while_loop}.
% \begin{itemize}
% \item[(i)] The current matching $M$ is maximal.
% \item[(ii)] For all $(u, v) \in E(G)$ such that $u \in V(M)$ and $v \in V(M)$, we have $(u, v) \in E^*$.
% \item[(iii)] For all $v \in V(M)$, we have $E_M(v) \cap E^* = E_M(v)$ or $|E^* \cap E_M(v)| \geq 2$.
% \end{itemize}

% % We obtain a maximal matching $M$ in Line \ref{line:quantum_matching_0}
% Obviously, the conditions (i)--(iii) hold at the beginning of the while loop.
% After we update the current matching $M$ along the $M$-augmenting path $P$ in Line \ref{line:quantum_matching_6}, two vertices $v_1, v_l$ are added to the set $V(M)$ and the sizes of sets $N_{v_2} \cap (V(G) \setminus V(M))$ and $N_{v_{l - 1}} \cap (V(G) \setminus V(M))$ decrease by $1$.
% The updated matching $M$ is maximal since there is no edge whose both endpoints are not in $V(M)$.
% After applying the procedure in Lines \ref{line:quantum_matching_update_start}--\ref{line:quantum_matching_update_end}, the conditions (ii) and (iii) satisfy.

% Now we present the following lemma, which is obtained by \cite[Lemma 5.6]{ben2019parameterized}.

% \begin{lemma}[{follows from Lemmas 5.6 in the arXiv version of \cite{ben2019parameterized}}] \label{lem:augmenting_path_find}
% If there exists an $M$-augmenting path in the input graph $G$, then there exists an $M$-augmenting path in the graph $(V, E^*)$.
% \end{lemma}

% For completeness, we provide a short proof of this lemma.

% \begin{proof}
% Fix some $M$-augmenting path $P$ in the input graph $G$, and denote by $V(P) = \{v_1, v_2, \ldots , v_{l - 1}, v_l\}$ the vertices in the path $P$.
% We have $v_1, v_l \in V(G) \setminus V(M)$, and $v_i \in V(M)$ for all $i \in [l] \setminus \{1, l\}$.
% By condition (ii), we have $(v_i, v_{i + 1}) \in E^*$ for all $i \in [l - 2] \setminus \{1\}$.
% % Since we have $(v_1, v_2) \in E(G)$ and $(v_{l - 1}, v_l) \in E(G)$, we have $|N_M(v_2)| \geq 1$ and $|N_M(v_{l - 1})| \geq 1$.
% Now $N_M(v_2)$ and $N_M(v_{l - 1})$ can not be empty.
% If $|N_M(v_2)| = |N_M(v_{l - 1})| = 1$, then we have $(v_1, v_2) \in E^*$ and $(v_{l - 1}, v_l) \in E^*$ by the condition (iii).
% Then we can find the path $P$ in the graph $(V, E^*)$.
% Otherwise, by the condition (iii), there exist two vertices $v_s, v_t \in V(G) \setminus V(M)$ such that $(v_s, v_2) \in E^*$ and $(v_{l - 1}, v_t) \in E^*$.
% Then, there exists an $M$-augmenting path $P'$ with vertex set $V(P') = \{v_s, v_2, \ldots, v_{l - 1}, v_t\}$ in the graph $(V, E^*)$. 
% \end{proof}

% By the condition (i), the size of the current matching $M$ is not maximum if and only if there exists an $M$-augmenting path in the input graph $G$.
% Then by Lemma \ref{lem:augmenting_path_find}, for the current matching $M$, there exists a matching $M'$ of size at least $|S| + 1$ if and only if there exists an $M$-augmenting path in the $(V, E^*)$.
% We note that the graph $(V, E^*)$ is a subgraph of the input graph $G$.
% This completes the proof of the correctness of \texttt{Quantum $k$-Matching}.
